Scalable Byzantine Consensus via Hardware-assisted Secret Sharing

The surging interest in blockchain technology has revitalized the search for effective Byzantine consensus schemes. In particular, the blockchain community has been looking for ways to effectively integrate traditional Byzantine fault-tolerant (BFT) protocols into a blockchain consensus layer allowing various financial institutions to securely agree on the order of transactions. However, existing BFT protocols can only scale to tens of nodes due to their $O(n^2)$ message complexity. In this paper, we propose FastBFT, a fast and scalable BFT protocol. At the heart of FastBFT is a novel message aggregation technique that combines hardware-based trusted execution environments (TEEs) with lightweight secret sharing primitives. Combining this technique with several other optimizations (i.e., optimistic execution, tree topology and failure detection), FastBFT achieves low latency and high throughput even for large scale networks. Via systematic analysis and experiments, we demonstrate that FastBFT has better scalability and performance than previous BFT protocols.

==> chapters/BFT_backup.tex <==
%!TEX root = ../submission.tex
\section{\BFT}
\label{sec:BFT}

In this section, we describe and analyze a full description of our solution, \BFT, the fastest BFT protocol to-date.


\subsection{Overview}

\BFT~is a new Byzantine fault-tolerant SMR service,
that guarantees safety in asynchronous network, but relies on weak synchrony for liveness.
In \BFT, we assume that each replica holds a $\TA$ that has a rollback-resistant memory\footnote{The rollback-resistant memory can be easily built using trusted counters}.
\BFT achieves its superior performance using a number of novel optimizations.

Similar to existing hardware assisted BFT protocols, \BFT~requires $n = 2f + 1$ replicas to tolerate $f$ (Byzantine) faults. However, unlike existing schemes, \BFT relies on TEEs (such as Intel SGX) for the purpose of generating and sharing secrets. That is, \BFT leverages functionalities from the TEE beyond trusted counters; \BFT still only involves TEEs in a limited way to ensure that it will not become a performance bottleneck.

\BFT assumes the optimistic model where $f+1$ active replicas agree and execute the requests
and the other $f$ passive just update their states. However, \BFT introduces an additional {\em preprocessing} phase to assist message aggregation and considerably reduces the message complexity in the {\em commit phase} when compared to existing BFT protocols (the {\em prepare} phase is exactly the same as other BFT protocols).

Namely, in the {\em commit} phase, all active replicas send their commit messages directly to the primary instead of all-to-all multicast.
Then the primary aggregates the commit messages and sends the result back. Figure~\ref{fig:FastBFT} depicts the message pattern of \BFT.



\begin{figure*}[t]
\centering
\begin{tikzpicture}
  [scale=.75,auto=center]
   \node at (0.9, 5.5) {\scriptsize \bf preprocessing};
   \node at (3, 5.5) {\scriptsize \bf request};
   \node at (5, 5.5) {\scriptsize \bf prepare};
    \node at (8, 5.54) {\scriptsize \bf commit};
     \node at (12, 5.5) {\scriptsize \bf reply};

   \draw [thick, dotted] (2, 0.5) -- (2, 6);
    \draw [thick, dotted] (4, 0.5) -- (4, 6);
     \draw [thick, dotted] (6, 0.5) -- (6, 6);
      \draw [thick, dotted] (10, 0.5) -- (10, 6);

   \node at (-0.5,5) {$\Cli$};
   \draw [thick] (0,5) -- (14,5);
   \draw [->,shorten >=2pt,>=stealth] (2.1, 5) -- (3.9, 4);

    \node at (-0.5,4) {$\Ser_p$};
     \draw [thick] (0,4) -- (14,4);
     \draw [->,shorten >=2pt,>=stealth] (0.6, 4) -- (1.9, 3);
     \draw [->,shorten >=2pt,>=stealth] (0.6, 4) -- (1.8, 2);

     \draw [->,shorten >=2pt,>=stealth] (4.1, 4) -- (5.8, 3);
     \draw [->,shorten >=2pt,>=stealth] (4.1, 4) -- (5.8, 2);

     \draw [->,shorten >=2pt,>=stealth] (8, 4) -- (9.8, 3);
     \draw [->,shorten >=2pt,>=stealth] (8, 4) -- (9.8, 2);

     \draw [->,shorten >=2pt,>=stealth] (12.1, 4) -- (13.8, 5);
  %   \draw [->,shorten >=2pt,>=stealth] (12.1, 4) -- (13.8, 3);
  %   \draw [->,shorten >=2pt,>=stealth] (12.1, 4) -- (13.8, 2);
     \draw [->,shorten >=2pt,>=stealth] (12.1, 4) -- (13.8, 1);

   \node at (-0.5,3) {$\Ser_1$};
   \draw [thick] (0,3) -- (14,3);

   \draw [->,shorten >=2pt,>=stealth] (6.3, 3) -- (7.8, 4);
    \draw [->,shorten >=2pt,>=stealth] (10.3, 3) -- (11.9, 4);

    \node at (-0.5,2) {$\Ser_2$};
     \draw [thick] (0,2) -- (14,2);

      \draw [->,shorten >=2pt,>=stealth] (6.3, 2) -- (7.9, 4);
     \draw [->,shorten >=2pt,>=stealth] (10.3, 2) -- (12.1, 4);

    \node at (-0.5,1) {$\Ser_3$};
    \node at (-0.5,0.6) {\scriptsize (passive)};
    \draw [thick] (0,1) -- (14,1);

\end{tikzpicture}
        \caption{Message pattern in FastBFT.}
        \label{fig:FastBFT}
\end{figure*}

Message aggregation is achieved in \BFT without using multisignature or any other public-key operations.
%so that replicas can get rid of the all-to-all broadcasts, and clients only need to receive and verify a single $\reply$.% (instead of $(f+1)$).
%A natural solution is using multisignature to aggregate the messages as CoSi~\cite{CoSi} did.
%However, there are two issues.
%The first one is that replicas need to sign different messages since they maintain different counter values, which thwart multisignature being used.
%To address this, we only have $\Ser_p$ use a trusted counter and have $\Ser_i$s record the latest counter value in their $\TA$s.
%As a result, all replicas maintain the same counter value.
%The second issue is that (multi)signature leads to larger message size and longer processing time.
%To get rid of this, we design a method that allows message aggregation without using any public key operations.
%We introduce a {\em preprocessing} phase, in which $\Ser_p$'s local $\TA$ generates a set of random secrets, and for each secret generates a commitment.
%Then it splits each secrets into shares and gives each share to each $\Ser_i$'s $\TA$.
%It also reveals the commitments to all replicas.
%Later in the commit phase, each $\Ser_i$ gets a share from its local $\TA$ and sends it to $\Ser_p$, which represents its $\commit$.
%After gathering enough shares, $\Ser_p$ reconstructs the secret and sends it to all $\Ser_i$s,
%which represents a threshold number of $\commit$s.
%Note that $\Ser_p$ cannot reconstruct the secret without gathering enough shares.
%We do the same thing for $\reply$.
%However, since the secrets are generated in the preprocessing phase, it is impossible to bind a secret with a request.
%Instead, we have $\Ser_p$'s TEE bind the secret with a counter value in the preprocessing phase,
%and bind that counter value with a request in the prepare phase.
%Thus, a request is bond with a specific secret.
Namely, in the preprocessing phase, the primary's local $\TA$ generates a set of random secrets and reveals a commitment (e.g., hash) for each secret.
Then, the TEE splits each secret into shares and distributes them to each active replica's $\TA$.
Later, in the prepare phase, the primary ties each request with a secret, and in the commit phase,
the primary gathers shares from active replicas and then reconstructs the secret, which represents an aggregate commit message.
%After gathering enough shares, $\Ser_p$ reconstructs the secret which represents a threshold number of commits, and sends it to all $\Ser_i$s.
Notice that the primary cannot reconstruct the secret without gathering enough shares.

However, since the secrets are generated in the preprocessing phase, a faulty primary can try to use the same secret for different requests---thus effectively performing equivocation.
To remedy this, we have the primary's TEE tie the secret with a monotonic counter value in the preprocessing phase,
and tie that counter value with a request in the prepare phase.
%Specifically, the commitment is generated from a counter value and a secret together.
%The $\prepare$ message that contains the request is signed with a specific counter value, and the $\commit$ message is the share corresponding to their counter value.
This ensures that each specific secret is tied with a single request.
To retrieve the share, an active replica is required to present its local $\TA$ a prepare message with a valid counter value, which will be recorded for further usage.
In this case,  only the primary uses a trusted counter and other replicas record the latest counter value in their $\TA$s as their ``trusted counters''.

This reduces the message complexity from $O(n^2)$ to $O(n)$.
In the {\em reply} phase, all active replicas again send their replies to the primary that aggregates the replies and returns it to the client as well as all passive replicas.
Thus, the client and passive replicas only need to receive one reply message instead of $f+1$.


%\noindent {\bf Tree topology.}
Even though this approach considerably reduces message complexity, the primary still needs to receive and aggregate $O(n)$ shares---which could lead to a bottleneck. This is exactly why \BFT requires the primary to organize the replicas into a spanning tree rooted at itself to distribute both communication and computation costs.
In this tree, the shares are propagated in a bottom-up process and each intermediate node aggregates its children's shares together with its own; finally, the primary only needs to receive and aggregate a small constant number of shares.
%This idea was proposed by Syta et al.~\cite{CoSi} and  used by Kokoris-Kogias et al.~\cite{ByzCoin} to improve the scalability of PBFT.
\remove{
However, the tree topology is fragile and will significantly reduce the robustness of the classical BFT,
because a faulty intermediate node makes its whole subtree appear to be ``faulty'', thus leading to more than $f$ ``failures''.
%Specifically, classical BFT (without a tree) can tolerate $f$ failures for free, whereas a single faulty replica in a tree may lead to more than $f$ ``failures''.
%In classical BFT, if a node receives no response from its children, it needs to contact its grandchildren, so on and so forth, which may incur serious time delay.
On the other hand, optimistic and speculative BFT require all (active) replicas to commit and execute the requests.
So their robustness does not degrade due to the use of a tree topology for communication.
%will not get any worse. %when using tree topology. % when a faulty intermediate node make its whole subtree ``faulty''.
}

%\noindent {\bf Failure detection.}
Finally, \BFT adapts a failure detection mechanism from \cite{BChain} to improve the robustness of the tree structure.
%Their mechanism is designed for a chain a replicas, and we adapt it to the tree structure.
Here, each node in the tree is allowed to flag its direct children (and only them) as potentially faulty.
%any node can suspect its direct children and only its direct children by sending a signed suspicion message up the tree.
A faulty node may simply crash or send a wrong share; when its parent detects this misbehavior, a signed ``suspect'' message will be sent up the tree.
%the crash fault by timeout and detects the Byzantine fault by verifying the share.
Upon receiving this message, the primary replaces the accused replica with a passive replica and puts the accuser in a leaf so that it cannot continue to accuse others.
%Recall that CheapBFT triggers a transition protocol to switch to MinBFT when suspected faulty replicas present.
%However, both the transition protocol and MinBFT are expensive, and MinBFT is not friendly to the tree structure.
%Instead of switching to MinBFT, we borrow the failure detection mechanism from BChain~\cite{BChain} to detect the faulty replica and replace it with a passive one.
%If $\Ser_p$ is faulty, all replicas will run a view-change operation to choose a new primary and a new set of active replicas.
%With failure detection,

In what follows, we describe the protocols of \BFT in greater details. In Section~\ref{sec:discussion}, we further put \BFT in perspective with a number of possible BFT variants.

\subsection{Protocol Specification (Normal case)}

\begin{figure}[h]
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]
\footnotesize
\Function{{\em preprocessing}($m$)}{}
\For{$1 \leq a \leq m$}
\State $c := c_{\textit{latest}}+a$ \Comment{$c_{\textit{latest}}$ is the latest counter value kept locally}
\State $s_c \overset{\$}{\leftarrow} \{0,1\}^l$
\State $h_c \leftarrow H(s_c, (c, v))$ \Comment{$v$ is the current view number kept locally}
\State $s_c^1 \oplus ... \oplus s_c^{f+1} \leftarrow s_c$   \Comment{splits $s_c$ into $f+1$ independent random secrets}
\For{each active replica $\Ser_i$}
\For{each of $\Ser_i$'s direct children: $\Ser_j$}
\State $\hat{h}_c^j= H(s_c^j\oplus_{k\in \phi_j}s_c^k)$  \Comment{$\phi_j$ is the set of $\Ser_j$'s descendants}
\EndFor
\State $\cipher_c^i \leftarrow E(k_i, \langle s_c^i, ( c,v), \{\hat{h}_c^j\}, h_c\rangle)$
\EndFor
\State $\langle h_c, ( c, v)\rangle_{\sigma_{p}} \leftarrow Sig(h_c, ( c, v))$ 
\EndFor 
\State \Return $\{\langle h_c, ( c, v) \rangle_{\sigma_{p}}, \{\cipher_c^i\}_i\}_c$
\EndFunction
\end{algorithmic}
\end{mdframed}
\label{alg:tee}
\caption{Pseudocode for $\TA$ interfaces.}
\end{figure}

%\ghassan{I more or less agree with the contents, but this is too much bullets to my taste. especially in setup and commit}
%\begin{enumerate}
%\ghassan{a nice figure would really help. It is typical in the distributed systems community to write pseudocode. I am neutral on this issue though.}
%\item \textbf{Setup:}
\noindent\textbf{Setup:}

\begin{itemize}
%\item Each client $\Cli$ sets up a shared secret key $k_{i}^{\Cli}$ with each $\Ser_i$.
\item $\Ser_p$'s local $\TA$ sets up a secret key $k_i$ with each $\Ser_i$'s local $\TA$.
\item $\Ser_p$ organizes active $\Ser_i$s into a balanced spanning tree.
\end{itemize}

%\item \textbf{Preprocessing:}
\noindent\textbf{Preprocessing:}
Following the current counter value, $\Ser_p$ chooses a set of unused counter values $\{c\}$.
For each counter value $c$, $\Ser_p$'s local $\TA$:

\begin{enumerate}

\item generates a random secret $s_c$ and calculates $h_c \leftarrow H(s_c, ( c, v))$, where $v$ is the current view number;

\item splits $s_c$ into $f+1$ independent random secrets: $s_c = s_c^1 \oplus ... \oplus s_c^{f+1}$;

\item for each active $\Ser_i$, calculates $e_c^i$ = $E(k_i, \langle s_c^i, ( c,v), \{\hat{h}_c^j\}, h_c\rangle)$,
where $E()$ is an authenticated encryption.
Suppose $\Ser_j$ is one of $\Ser_i$'s direct children, $\hat{h}_c^j$ is calculated as $\hat{h}_c^j= H(s_c^j\oplus_{k\in \phi_j}s_c^k)$,
where $\phi_j$ is the set of $\Ser_j$'s descendants;
%$h_i^j= \oplus_{k\in \phi_i}s_k^j$ where $\phi_i$ is the set of $\Ser_i$'s descendants.

\item calculates $\langle h_c, ( c, v)\rangle_{\sigma_{p}}$ which is a signature generated using the signing key inside $\TA$;

\item gives $\langle h_c, ( c, v) \rangle_{\sigma_{p}}$ and $\{e_c^i\}$ to $\Ser_p$.

\end{enumerate}

$\Ser_p$ sends $e_c^i$ to each active replica $\Ser_i$. %and sends $\langle h^j, c^j\rangle_{\sigma_{p}}$ to all passive replicas.
It can send these messages in a batch for all counter values.

%\item \textbf{Request:}
\noindent\textbf{Request:}
$\Cli$~requests the execution of $op$ by sending a request message $M = \langle \request, op \rangle_{\sigma_{\Cli}}$ only to $\Ser_p$, where $\sigma_{\Cli}$ is $\Cli$'s signature.
If $\Cli$ receives no reply before a timeout, it multicasts $M$ to all replicas.

%\item \textbf{Prepare:}
\noindent\textbf{Prepare:}
$\Ser_p$ multicasts $\langle \prepare, M, \langle H(M), ( c, v) \rangle_{\sigma_{p}}\rangle$ to all active $\Ser_i$s
\footnote{It can either send it along the tree or multicasts directly, depending on the underlying network.}.
%where $M$ is the $\request$ message, $v$ indicates the view number, and
$\langle H(M), (c, v)\rangle_{\sigma_{p}}$ is returned by $\Ser_p$'s local $\TA$, where $c$ is the current counter value.
We say that the request message $M$ has been {\em prepared} at this point.

%\item \textbf{Commit:}
\noindent\textbf{Commit:}
Each active $\Ser_i$ verifies $\Cli$'s signature in $M$ and then gives $\langle H(M), (c, v) \rangle_{\sigma_{p}}$ and the corresponding $e_c^i$ to its local $\TA$, which verifies:
\begin{itemize}
\item the validity of $\sigma_{p}$;
\item the integrity of $e_c^i$;
\item whether the counter value and view number inside $e_c^i$ is equal to $(c, v)$;
\item whether the latest counter value recorded by itself is $c-1$.
\end{itemize}
If these verifications succeed, $\TA$ records $c$ as the latest counter value in its memory and reveals the result $\langle s_c^i, (c, v), \{\hat{h}_c^j\}, h_c\rangle$ to $\Ser_i$.

$\Ser_i$ waits to receive a partial aggregate share $\hat{s}_c^j$ from each of its immediate children $\Ser_j$ and verifies if $H(\hat{s}_c^j) = \hat{h}_c^j$.
If this verification succeeds, $\Ser_i$ calculates its own response $\hat{s}_c^i = s_c^i \oplus_{j\in \phi_i} \hat{s}_c^j$, and sends it to its parent.

After receiving the valid aggregate shares, $\Ser_p$ reconstructs $s_c$ and checks it against $h_c$.
If valid, $\Ser_p$ executes $op$ and get the result $res$.
Then it multicasts $\langle \commit, s_c, res, $ $\langle H(M||res), (c+1, v)\rangle_{\sigma_{p}}\rangle$
\footnote{The counter value here does not necessary to be $c+1$, since $\Ser_p$ may process other requests concurrently while waiting for the shares of $s_c$. We use $c+1$ here for simplicity.}
to all active $\Ser_i$s.
We say that $M$ has been {\em committed} at this point.

%\item \textbf{Reply:}
%\noindent\textbf{Execute:}

%Upon receiving a valid $s^j$, each active server $\Ser_i$ sends
%a reply $E(k_i^{\Cli}, \langle \reply, res  \rangle)$ to $\Cli$ and a state update $\langle \update, res,  s^j  \rangle$ to all passive servers.

%\item \textbf{Update:}
\noindent\textbf{Reply:} %\ghassan{This part is hard to follow/parse. Could you please go over it again?}
Upon receiving $s_c$, each active $\Ser_i$ also verifies it against $h_c$,
after which active $\Ser_i$s execute $op$ and get the result $res$.
They execute a procedure similar to the commit phase in order to open $s_{c+1}$.
$\Ser_p$ sends $\langle \reply, M, s_c,  \langle h_c, (c,v) \rangle_{\sigma_{p}}, \langle H(M), (c,v) \rangle_{\sigma_{p}}, res, s_{c+1}, $ $\langle h_{c+1}, (c+1,v) \rangle_{\sigma_{p}}, \langle H(M||res), (c+1, v)\rangle_{\sigma_{p}}\rangle$ to $\Cli$ as well as all passive replicas.
We say that $M$ has been {\em replied} at this point.
$\Cli$ verifies the validity of this message:
\begin{enumerate}
\item A valid $\langle h_c, (c, v) \rangle_{\sigma_{p}}$ represents the fact that $(c,v)$ has been tied to a secret $s_c$ whose hash is $h_c$.
\item A valid $\langle H(M), (c,v) \rangle_{\sigma_{p}}$ represents the fact that $(c,v)$ has been tied to the request message $M$.
\item Thus, $M$ has been tied to $s_c$ based on 1) and 2).
\item A valid $s_c$ (i.e., $H(s_c, (c, v)) = h_c$) represents the fact that all active replicas have agreed to execute the operation in $M$ with counter value $c$.
\item A valid $s_{c+1}$ denotes the fact that all active replicas have executed the operation in $M$.
\end{enumerate}
Each passive replica performs this verification, executes the operation in $M$,
and transfers the reply message to its local $\TA$ in order to update the latest counter value.


%After receiving $f+1$ valid $\update$s, the passive replica adjusts its application state by processing the sate update.

%\end{enumerate}


\subsection{Failure detection}
%\ghassan{You need to specifically discuss that any failure above will trigger failure detection to occur. It is not only about timeouts. If somebody send the wrong hash, then I guess you have to initiate failure detection, no?}

To improve the robustness of \BFT, we introduce a failure detection mechanism to detect and recover from non-primary faults.
Here, crash faults are detected by timeout and the Byzantine faults are detected by verifying the share.


Specifically, upon receiving and sending a $\prepare$/$\commit$ message, $\Ser_i$ starts a timer for each of its direct children.
If $\Ser_i$ fails to receive a share from $\Ser_j$ before the timer expires or if $\Ser_i$ receives a wrong share that does not match $\hat{h}_c^j$,
it sends $\langle \suspect, \Ser_j \rangle$ to both $\Ser_p$ and its parent to signal a failure of $\Ser_j$.
%Otherwise, it just cancels the timer for $\Ser_j$.
Whenever a replica receives a $\suspect$ message from its children, the message is forwarded to its parent along the tree until it reaches the root.

By passing the message along the tree, parent nodes cancel timers; this process also reduces the number of $\suspect$ messages.
If $\Ser_p$ receives multiple $\suspect$ messages along the same path, the one that is closest to the leaf is only handled.

Upon receiving a $\suspect$ message,
$\Ser_p$ multicasts $\langle \newtree, T, T', \langle H(T||T'), (c, v)\rangle_{\sigma_{p}} \rangle$ to all replicas,
where $T$ is the old tree and $T'$ the the new tree.
This message basically replaces the accused replica $\Ser_j$ with a randomly chosen passive replica and moves the accuser $\Ser_i$ to a leaf position.
The rationale for moving $\Ser_i$ is to prevent it from constantly accusing others if it is faulty.

Notice that this approach allows a Byzantine $\Ser_p$ to evict correct replicas on purpose.
However, there always will be at least one correct replica among the $f+1$ active replicas. %{\color{red}please explain why.}

Notice that if there are multiple faulty nodes along the same path, the current mechanism can only detect one failure within one round.
We can extend this mechanism by having $\Ser_p$ check the correctness of all active replicas individually after one failure detection to allow the detection of multiple failures within one round.
%However, it becomes trickier if there are multiple Byzantine faulty nodes along the same path.

\begin{figure}[p]
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]
\footnotesize
\State \textbf{upon} invocation of PREPROCESSING at $\Ser_p$ \textbf{do}
\State ~~~~ decide the number of counters $m$ to be preprocessed
\State ~~~~ $\{\langle h_c, ( c, v) \rangle_{\sigma_{p}}, \{\cipher_c^i\}_i\}_c$ $\leftarrow$ $\TA$.{\em preprocessing}($m$)
\State ~~~~ \textbf{for} each active $\Ser_i$ \textbf{do}
\State ~~~~~~~~send $\{\cipher_c^i\}_c$ to $\Ser_i$
\\
\State \textbf{upon} reception of $M = \langle \request, op \rangle_{\sigma_{\Cli}}$ at $\Ser_p$ \textbf{do}
\State ~~~~ verify $\sigma_{\Cli}$
\State ~~~~ $\langle H(M), ( c, v) \rangle_{\sigma_{p}}$ $\leftarrow$ $\TA$.{\em request\_counter}($H(M)$)
\State ~~~~ send $\langle \prepare, M, \langle H(M), ( c, v) \rangle_{\sigma_{p}}\rangle$ to active $\Ser_i$s 
\\
\State \textbf{upon} reception of $\langle \prepare, M, \langle H(M), ( c, v) \rangle_{\sigma_{p}}\rangle$ at $\Ser_i$ \textbf{do}
\State ~~~~  $\langle s_c^i, (c, v), \{\hat{h}_c^j\}, h_c\rangle$ $\leftarrow$ $\TA$.{\em verify\_counter}($\langle H(M), ( c, v) \rangle_{\sigma_{p}}$, $\cipher_c^i$)
\State ~~~~ $\hat{s}_c^i := s_c^i$
\State ~~~~  \textbf{if} $\Ser_i$ is a leaf node \textbf{do}
\State ~~~~~~~~ send $s_c^i$ to its parent
\State ~~~~ \textbf{else} \textbf{do}
\State ~~~~~~~~ set timers for its direct children
\\
\State \textbf{upon} timeout of $\Ser_j$'s share at $\Ser_i$ \textbf{do}
\State ~~~~ send $\langle \suspect, \Ser_j \rangle$ to both $\Ser_p$ and its parent
\\
\State \textbf{upon} reception of $\langle \suspect, \Ser_k \rangle$ from $\Ser_j$ at $\Ser_i$ \textbf{do} 
\State  ~~~~  \textbf{if} $\Ser_i$ is the primary
\State  ~~~~~~~~ generate a new tree structure $T'$ s.t., $\Ser_k$ is replaced with a passive replica and $\Ser_j$ is placed in the leaf
\State  ~~~~~~~~ $\langle H(T||T'), (c, v)\rangle_{\sigma_{p}} \rangle$ $\leftarrow$ {\em request\_counter}($H(T||T')$)
\State  ~~~~~~~~ send $\langle \newtree, T, T', \langle H(T||T'), (c, v)\rangle_{\sigma_{p}} \rangle$ to all replicas
\State  ~~~~ \textbf{else} \textbf{do} 
\State  ~~~~~~~~ cancel the timer for $\Ser_j$
\State  ~~~~~~~~ forward the $\suspect$ message to its parent node 
\\
\State \textbf{upon} reception of $\hat{s}_c^j$ at $\Ser_i$ \textbf{do}
\State ~~~~  \textbf{if} $H(\hat{s}_c^j) = \hat{h}_c^j$ \textbf{do}
\State ~~~~~~~~ $\hat{s}_c^i := \hat{s}_c^i \oplus \hat{s}_c^j$
\State ~~~~  \textbf{else} \textbf{do} 
\State ~~~~~~~~  send $\langle \suspect, \Ser_j \rangle$ to both $\Ser_p$ and its parent
\\
\State ~~~~  \textbf{if} $\Ser_i$ has received all $\{\hat{s}_c^j\}_j$ and no $\suspect$ message sent
\State ~~~~~~~~  send $\hat{s}_c^i$ to its parent
\\
\State \textbf{upon} reception of  $\{\hat{s}_c^i\}$ at $\Ser_p$ \textbf{do} 
\State ~~~~ $s_c := s_c^p$
\State ~~~~ \textbf{for} each $\hat{s}_c^i$ \textbf{do}
\State ~~~~~~~~ \textbf{if} $H(\hat{s}_c^i) = \hat{h}_c^i$ \textbf{do}
\State ~~~~~~~~~~~~ $s_c := s_c \oplus \hat{s}_c^i$
\State ~~~~~~~~ \textbf{else}  \textbf{do}
\State ~~~~~~~~~~~~ replace $\Ser_i$ with a passive node
\State ~~~~~~~~~~~~ \textbf{return}
\State ~~~~ \textbf{if} $s_c$ is for commit \textbf{do}
\State ~~~~~~~~ $res$ $\leftarrow$ execute $op$
\State ~~~~~~~~ $\langle H(M||res), (c', v) \rangle_{\sigma_{p}}$ $\leftarrow$ $\TA$.{\em request\_counter}($H(M||res)$)
\State ~~~~~~~~ send $\langle \commit, s_c, res, \langle H(M||res), (c', v) \rangle_{\sigma_{p}}\rangle$ to active $\Ser_i$s 
\State ~~~~ \textbf{else if} $s_c$ is for reply \textbf{do}
\State ~~~~~~~~ sends $\langle \reply, M, s_{c'},  \langle h_{c'}, (c',v) \rangle_{\sigma_{p}}, \langle H(M), (c',v) \rangle_{\sigma_{p}}, res,$ 
$s_{c},\langle h_{c}, (c,v) \rangle_{\sigma_{p}}, \langle H(M||res), (c, v)\rangle_{\sigma_{p}}\rangle$ to $\Cli$ and passive replicas.
\\
\State \textbf{upon} reception of $\langle \commit, s_c, res, \langle H(M||res), (c, v) \rangle_{\sigma_{p}}\rangle$ at $\Ser_i$ \textbf{do}
\State ~~~~  $\langle s_c^i, (c, v), \{\hat{h}_c^j\}, h_c\rangle$ $\leftarrow$ $\TA$.{\em verify\_counter}($\langle H(M), ( c, v) \rangle_{\sigma_{p}}$, $\cipher_c^i$)
\State ~~~~ $\hat{s}_c^i := s_c^i$
\State ~~~~  \textbf{if} $\Ser_i$ is a leaf node \textbf{do}
\State ~~~~~~~~ send $s_c^i$ to its parent
\State ~~~~ \textbf{else} \textbf{do}
\State ~~~~~~~~ set timers for its direct children
\\
\State \textbf{upon} reception of $reply = \langle \reply, M, s_{c'},  \langle h_{c'}, (c',v) \rangle_{\sigma_{p}}, $ 
$\langle H(M), (c',v) \rangle_{\sigma_{p}}, res, s_{c},\langle h_{c}, (c,v) \rangle_{\sigma_{p}}, \langle H(M||res), (c, v)\rangle_{\sigma_{p}}\rangle$ at $\Ser_i$ \textbf{do}
\State ~~~~ $\TA$.{\em update\_counter}($reply$)
\end{algorithmic}
\end{mdframed}
\label{fig:normal_case}
\caption{Pseudocode for Normal case with failure detection.}
\end{figure}

\subsection{View-change}

If a replica receives a valid client request but receives no response (or invalid messages) from $\Ser_p$ after a timeout,
it can suspect that $\Ser_p$ is faulty and initializes a view-change as follows:

\begin{enumerate}
\item $\Ser_i$ multicasts $\langle \reqviewchange,  v, v' \rangle$ to all replicas. %$\UI_p$ is included in this message as a proof for primary's mis-behaviour.

\item After receiving $f+1$ $\reqviewchange$ messages, each $\Ser_i$ multicasts $\langle \viewchange, O,$ $\langle H(O), (c,v) \rangle_{\sigma_{i}} \rangle$ to all replicas,
where $c$ is a counter value following the latest counter value recorded by its local $\TA$,
and $O$ is a set that includes all $\request$, $\prepare$, $\commit$ and $\reply$ messages it has received since the latest checkpoint\footnote{Like other BFT protocols,
\BFT also generates checkpoints periodically to limit the number of messages in the log. We skip this description due the the page limit.}.
At this point, $\Ser_i$ stops accepting messages for $v$.

\item After receiving $f+1$ $\viewchange$ messages, the new primary $\Ser_{p'}$ (that satisfies $p' = v'$ mod $n$)
multicasts $\langle \newview, L, T, \langle H(L||T), (c+1, v), (c', v') \rangle_{\sigma_{p'}} \rangle$,
where $L$ is the set of requests that were prepared/committed/replied during this view ($L$ is constructed based on all the $O$s it has received),
$T$ is the new tree for view $v'$ that specifies the set of $f+1$ new active replicas denominated by $\Ser_{p'}$,
and $c'$ is the initial counter value for view $v'$.

\item After receiving the $\newview$ message from $\Ser_{p'}$, $\Ser_i$ verifies if $L$ was constructed properly doing the same operation as $\Ser_{p'}$.
Subsequently, $\Ser_i$ begins the new view $v'$ after executing all requests in $L$ that have not yet been executed locally, following the counter values.

\item The new set of active replicas run the pre-processing phase for view $v'$, and then reply to the clients' requests that have not been replied yet, and process the requests that have not been prepared yet.
%\ghassan{you need to discuss the case where faulty nodes try to evict correct nodes on purpose.}
\end{enumerate}

\begin{figure}[h]
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]
\footnotesize

\State \textbf{upon} timeout of $\Ser_p$'s $\prepare$ message at $\Ser_i$ \textbf{do}
\State ~~~~ send $\langle \reqviewchange,  v, v' \rangle$ to all replicas
\\
\State \textbf{upon} reception of $f+1$ $\langle \reqviewchange,  v, v' \rangle$ messages at $\Ser_i$ \textbf{do}
\State ~~~~ construct $O$ based on all $\request$, $\prepare$, $\commit$ and $\reply$ messages it has received since the latest checkpoint. 
\State ~~~~ $\langle H(O), (c, v) \rangle_{\sigma_{p}}$ $\leftarrow$ $\TA$.{\em request\_counter}($H(O)$)
\State ~~~~ sends $\langle \viewchange, O,$ $\langle H(O), (c,v) \rangle_{\sigma_{i}} \rangle$ to all replicas
\\
\State \textbf{upon} reception of $f+1$ $\langle \viewchange, O,$ $\langle H(O), (c,v) \rangle_{\sigma_{i}} \rangle$ messages at $\Ser_{p'}$ \textbf{do}
\State ~~~~ construct $L$ based on all $O$s it as received
\State ~~~~ choose $f+1$ new active replicas $\{\Ser_i\}$ and construct a new tree $T$
\State ~~~~ $\{\omega_i\}$ $\leftarrow$ $\TA$.{\em request\_keys}($\{\Ser_i\}$)
\State ~~~~ $\langle H(L||T), ( c, v) \rangle_{\sigma_{p'}}$ $\leftarrow$ $\TA$.{\em request\_counter}($H(L||T)$)
\State ~~~~ send $\langle \newview, L, T, \langle H(L||T), (c, v) \rangle_{\sigma_{p'}}, \{\omega_i\} \rangle$ to all replicas
\State 
\State \textbf{upon} reception of $\langle \newview, L, T, \langle H(L||T), (c, v) \rangle_{\sigma_{p'}}, \{\omega_i\} \rangle$ at $\Ser_{p'}$ \textbf{do}
\State ~~~~ \textbf{if} $L$ was constructed \textbf{do} 
\State ~~~~~~~~ execute all requests in $L$ that have not yet been executed locally
\State ~~~~~~~~ $\TA$.{\em set\_key}($\omega_i$)
\end{algorithmic}
\end{mdframed}
\label{fig:view_change}
\caption{Pseudocode for view-change.}
\end{figure}



\remove{
\begin{enumerate}
\item The suspecting replica sends a $\langle \panic  \rangle$ message to all other replicas, who react by rebroadcasting the message to ensure that all replicas are notified.
\item The new primary $\Ser_{p'}$ is chosen deterministically as the active replica with the lowest id apart from $\Ser_p$.
$\Ser_{p'}$ sends $\langle \history, $ $O, $ $\langle H(O), c \rangle_{\sigma_{p'}} \rangle$ to all replicas, where $c$ is a counter value following the latest counter value recorded by its local $\TA$, and $O$ is the {\em abort history} that includes all $\request$s, $\prepare$s, $\commit$s and $\reply$s it has received during this view.
%\begin{itemize}
%\item $\reply$s for the executed requests;
%\item $\commit$s for the committed requests;
%\item $\prepare$s for the prepared requests;
%\item $\request$s for the requests that receives no $\prepare$s.
%\end{itemize}
\item When $\Ser_i$ receives $\history$ from $\Ser_{p'}$, it verifies the counter values in $O$ first, and then sends $\langle \viewchange, $ $H(O), \langle H(O), c \rangle_{\sigma_{i}} \rangle$.
When a replica has obtained a correct history and $f+1$ matching $\viewchange$ messages, the history becomes stable.
In this case, the replica processes the abort history, taking into account its local state.
Having processed the history, all non-faulty replicas are in a consistent state and therefore able to safely switch to the new view.

\item After receiving $f+1$ $\viewchange$s, $\Ser_{p'}$ broadcasts $\langle \newview, $ $R, $ $\langle H(R), (c+1) \rangle_{\sigma_{p'}} \rangle$, where $R$ is the set of $f+1$ new active replicas denominated by $\Ser_{p'}$. \ghassan{you mean max(c)+1?}
\end{enumerate}
}



\subsection{Application to Classical BFT Protocols}

In the previous paragraphs, we described the protocol specification of FastBFT assuming the optimistic paradigm.
In what follows, we demonstrate that our message aggregation technique is applicable to other trusted counter based BFT protocols as well.
Unlike speculative or optimistic BFT where all (active) replicas are required to commit and/or reply, classical BFT only requires $f+1$ replicas to commit and reply. 
When applying our techniques to classical BFT models, this means that one needs to use a ($f+1$)-out-of-$n$ secret sharing technique, such as Shamir's polynomial-based secret sharing, rather than the $n$-out-of-$n$ XOR secret sharing.
%we have to use a Shamir's threshold secret sharing~\cite{} instead of simply splitting the secret using XOR.
%To do so, we propose the following instantiation. {\color{red}it would be good to remind readers here of the system model of MinBFT.}

We take MinBFT~\cite{MinBFT} as an example to explain the idea. 
In MinBFT, $\Ser_p$ sends a $\prepare$ message including a monotonic counter value to all replicas. 
Then, each $\Ser_i$ multicasts a $\commit$ message to others to agree on the proposal from $\Ser_p$. 
To get rid of this all-to-all multicast, we again introduce a preprocessing phase, 
where $\Ser_p$'s local $\TA$ first generates $n$ random values $x_1, ..., x_n$, and, for each $x_i$, computes $y_i = \prod_{j\neq i}\frac{x_j}{x_j-x_i}$. Then, for each counter value $c$, $\Ser_p$ performs the following operations:
\begin{enumerate}

\item $\Ser_p$ generates a polynomial with independent random coefficients: $f_c(x) = s_c + a^1_cx^1 + ... + a^f_cx^f$ where $s_c$ is a secret to be shared.

\item $\Ser_p$ calculates $h_c \leftarrow H(s_c, (c,v))$.

\item For each active $\Ser_i$, $\Ser_p$ calculates $e_c^i$ = $E(k_i, \langle (x_i, f_c(x_i)), (c,v), \{\hat{h}_c^j\}, h_c\rangle)$.
Suppose $\Ser_j$ is one of $\Ser_i$'s direct children, $\hat{h}_c^j$ is calculate as $\hat{h}_c^j= H(f_c(x_j)y_j+\sum_{k\in \phi_j}f_c(x_k)y_k)$,
where $\phi_j$ is the set of $\Ser_j$'s descendants.

\item $\Ser_p$ calculates $\langle h_c, (c, v)\rangle_{\sigma_{p}}$ which is a signature generated using the signing key inside $\TA$.

\item $\Ser_p$ gives $\langle h_c, (c, v)\rangle_{\sigma_{p}}$ and $\{e_c^i\}$ to $\Ser_p$.
\end{enumerate}
Subsequently, $\Ser_p$ sends $e_c^i$ to each replica $\Ser_i$.
Later on, in the commit phase, after receiving at least $f+1$ shares, $\Ser_p$ reconstructs the secret: $s_c = \sum_{i=1}^{f+1}f_c(x_i)y_i$.

%{\color{red}please say that briefly why this satisfies the liveness and safety conditions as mentioned before.}
%\jianliu{Now, the proof is after this. Is this comment still valid?}
%{\color{red}i like this section, but it is hard to follow. I would start from the ``synthesis and comparison of design choices''. I would outline the full scope to readers. Then, i would tell readers that if they want a more robust scheme, here is how our optimization techniques can be built atop MinBFT. Do you follow me?}



==> chapters/discussions_backup.tex <==
%!TEX root = ../submission.tex
\section{BFT \`A la Carte}
\label{sec:discussion}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[Components. \emph{*Not all combinations are possible, e.g., L is not applicable to C}]{
        \label{fig:components}
        \includegraphics[width=0.4\textwidth]{./pic/modules}}
    \end{subfigure}
    \begin{subfigure}[Comparisons of design choices.]{
        \label{fig:comparisons}
        \includegraphics[width=0.4\textwidth]{./pic/comparisons}} 
    \end{subfigure}
    \caption{Components and design choices.\TODO{correct the refs, linear to XOR} }
    \vspace{-1.5em}
\end{figure*}

In this section, we give synthesis and comparisons of different BFT design choices. To this end, we categorize BFT protocols based on their message patterns, reliance on secure hardware, and message aggregation techniques. 
\fig{fig:components} depicts these design choices for constructing BFT protocols.
%As depicted in Fig.~\ref{fig:components}, we have the following design choices.


%Here, we group BFT protocols in three basic models based on their message patterns, reliance on secure hardware, and message aggregation techniques.
%\vspace{0.5 em}
\noindent \textbf{Model: }As mentioned in Section~\ref{sec:Background}, we distinguish between three possible models:
the classical model (C) (e.g., PBFT~\cite{PBFT}),
the optimistic model (O) (e.g., Yin et. al~\cite{Yin}),
and the speculative model (S) (e.g., Zyzzyva~\cite{Zyzzyva}). Secure hardware (H) can be used in conjunction with all three models. For instance, MinBFT~\cite{MinBFT} combines
the classical model (C) and secure hardware (H); to ease presentation, we say that MinBFT belongs to the CH family. Similarly, CheapBFT~\cite{CheapBFT} and MinZyzzyva~\cite{MinBFT} belong to OH (i.e., combine the optimistic model with secure hardware), and SH (i.e., combine the speculative model with secure hardware), respectively.

%\vspace{0.5 em}
\noindent \textbf{Message Aggregation: }One can further extend these constructs by leveraging message aggregation. Here, we distinguish between message aggregation based on multisignatures (M) such as~\cite{CoSi} and secret-sharing techniques (such as the one used in \BFT). We further classify secret-sharing techniques into (the more efficient) XOR-based schemes (X) which are used in \BFT, and (the less efficient) polynomial-based secret-sharing techniques (P). Notice that secret-sharing techniques are only applicable to hardware-assisted BFT protocols (i.,e to CH, OH, and SH). Furthermore, in the CH model, only polynomial-based secret-sharing techniques can only be used since classical BFT only requires a threshold number of replicas in the commit and reply phases. On the other hand, XOR-based secret-sharing techniques can be used in conjunction with \mbox{OH and SH}.

%\vspace{0.5 em}
\noindent \textbf{Optimized topology: } In addition, we can apply the tree topology with failure detection (T) to any of the above combinations e.g., CHPT, OHXT (which is \BFT), SHXT and CMT (which is ByzCoin).


\subsection*{Comparison}

In \fig{fig:comparisons}, we compare the aforementioned design choices according to two dimensions:
\begin{itemize}
\item {\bf Performance:} This mainly refers to the latency required to complete a request and to the peak throughput exhibited by the system in the normal case;
\item {\bf Resilience:} This refers to the cost required to recover from non-primary faults\footnote{All BFT protocols require view-change to recover from primary faults,
and this operation takes similar cost among different protocols.
So we only consider non-primary faults in terms of resilience.}. 
\end{itemize}


Clearly, speculative BFT protocols (S) provide the best performance among the considered message patterns since it avoids all-to-all multicast.
However, speculative execution cannot tolerate even a single crash fault and the client needs to help correct replicas to converge on a single ordering of requests.
In real-world scenarios, clients may have neither incentives nor resources (e.g., lightweight clients) to do so.
If a (faulty) client fails to report the inconsistency, replicas whose state has diverged from others may not discover this.
Moreover, if inconsistency appears, replicas may have to rollback some executions, which makes the programming model more complicated.
Therefore, speculative BFT performs the worst in terms of resilience.
In contrast, classical BFT protocols (C) can tolerate non-primary faults for free but requires all replicas to be involved in the agreement stage.
By doing so, these protocols achieve the best resilience but at the expense of bad performance.
Optimistic BFT protocols~(O), on the other hand, achieve a solid tradeoff between performance and resilience. These protocols only require active replicas to execute the agreement protocol which significantly reduces message complexity but still requires all-to-all multicast.
Although these protocols requires a transition protocol or view change to tolerate non-primary faults, they require neither support from the clients nor any rollback mechanism. %and there is no need of rollback.

Message aggregation significantly increase performance of optimistic BFT and classical BFT protocols but is of little help to speculative BFT which exhibits $O(n)$ message complexity. %message complexity is $O(n)$ already.

The tree topology improves the performance of all protocols. %dimension of speculative BFT (SHXT) and classical BFT (CHPT).
For SHXT, the resilience remains the same as before, since it still requires to do rollback if failure happens.
For CHPT, the resilience will be reduced to almost the same level with OHXT, since a faulty node in the tree can make its whole subtree ``faulty'', thus it requires failure detection (the \mbox{same as OHXT)}. 

As shown in Fig.~\ref{fig:comparisons}, \BFT achieves good resilience and very high performance guarantees. Indeed, the reliance on hardware security mechanisms and XOR-based secret-sharing considerably bridge the performance gap between optimistic and speculative BFT protocols and not adversely impact resilience. \BFT additionally leverages a tree topology with failure detection in order to further boost the system's performance and resilience. We confirm this analysis by means of experimental evaluation in the following section.

\remove{
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{./pic/modules} % first figure itself
    \caption{Synthesis and comparisons of design choices.}
    \label{fig:synthesis}
    \emph{A note}
\end{figure*}
}

\remove{
\begin{SCfigure}
	\label{fig:modules}
        \includegraphics[scale=0.48]{./pic/modules}
        \caption{\footnotesize{Different combinations:} \\
 {\scriptsize Classic BFT+(1)=MinBFT \\
Optimistic BFT + (1) = CheapBFT \\
Speculative BFT + (1) = MinZyzzyva \\
MinBFT + (2.1) = MinAggre \\
CheapBFT + (2.2)  = CheapAggre \\
MinZyzzyva + (2.2) = MinZAggre \\
MinAggre + (3.1) = MinAggreTree  \\
CheapAggre + (3.1)= \BFT \\
MinZAggre + (3.1) = MinZAggreTree  \\
Classic BFT + (2.3) + (3.1) = CoSi \\}
}
\end{SCfigure}
\begin{figure}[t]
	\centering
        \centerline{\includegraphics[scale=0.57]{./pic/comparisons}}
        \caption{Comparison between different combinations.}
        \label{fig:comparisons}
\end{figure}
}




==> chapters/performance_backup.tex <==
%!TEX root = ../submission.tex
\section{Performance Evaluation}
\label{sec:performance}

\begin{figure*}[htbp]
  \centering

     \subfigure[CPU time vs number of replicas in the pre-processing phase.
     ]{
          \label{fig:8}
          \includegraphics*[width=0.32\linewidth]{plot/T5-preprocess-vs-n.pdf}}
          \subfigure[Latency vs the payload size.
     ]{
         \label{fig:7}
         \includegraphics*[width=0.32\linewidth]{plot/T4-latency-vs-payload_n103.pdf}}
         \subfigure[Latency vs throughput for payload size=1024KB and $f=51$.
     ]{
          \label{fig:3}
          \includegraphics*[width=0.32\linewidth]{plot/T3-latency-vs-tp_f51_1024.pdf}}\\
           \subfigure[Latency vs throughput for payload size=1MB and $f=51$.
     ]{
          \label{fig:6}
          \includegraphics*[width=0.32\linewidth]{plot/T3-latency-vs-tp_f51_1048576.pdf}}
      %        \hspace{.01in}
     %          \hspace{.01in}
          \subfigure[Peak throughput vs number of replicas.\TODO{y-axis to peak throughput}
     ]{
          \label{fig:9}
          \includegraphics*[width=0.32\linewidth]{plot/T6-tp-vs-n.pdf}}
   \subfigure[Latency vs $f$ for payload size=1024KB.
     ]{
          \label{fig:1}
          \includegraphics*[width=0.32\linewidth]{plot/T1-latency-vs-f_1024.pdf}}\\
        %   \hspace{.01in}
     \subfigure[Peak throughput $f$ for payload size=1024KB.\TODO{y-axis to peak throughput}
     ]{
          \label{fig:2}
          \includegraphics*[width=0.32\linewidth]{plot/T2-tp-vs-f_1024.pdf}}
    % \hspace{.01in}
      %     \hspace{.01in}\\
     \subfigure[Latency vs $f$ for payload size=1MB.
     ]{
         \label{fig:4}
         \includegraphics*[width=0.32\linewidth]{plot/T1-latency-vs-f_1048576.pdf}}
      %        \hspace{.01in}
     \subfigure[Peak throughput $f$ for payload size=1MB.\TODO{y-axis to peak throughput}
     ]{
          \label{fig:5}
          \includegraphics*[width=0.32\linewidth]{plot/T2-tp-vs-f_1048576.pdf}}
     %          \hspace{.01in}
     \caption{Evaluation Results. Data points are averaged over 1500 runs; where appropriate, we include the corresponding 95\% confidence intervals.}
    \label{fig:results}
    \vspace{-1.5em}
\end{figure*}

In this section, we implement and evaluate the performance of \BFT in comparison to PBFT~\cite{PBFT}, Zyzyva~\cite{Zyzzyva}, MinBFT~\cite{MinBFT} and CheapBFT~\cite{CheapBFT}.
%We also analyze the performance of a variant of MinBFT, dubbed MinAgree, that leverages our secret-sharing-based message aggregation scheme.

\subsection{Experimental Setup and Methodology}

Our implementation is based on Golang. In our implementation, we relied on SHA256 for hashing purposes, 256-bit keyed HMACs to implement MACs, 2048-bit RSA to generate RSA signatures.% and Elliptic curve F to implement BLS signatures.


We deployed our BFT implementations on a private network consisting of five 8 vCore Intel Xeon E3-1240 equipped with 32 GiB RAM and Intel SGX.
All the BFT nodes were running in separate processes on theses machine. At all times, we load balance the number of BFT nodes spawned on each machine; we spawned a maximum of 200 processes (emulating BFT nodes) on the 5 machines. The clients were running on a 8 vCore Intel Xeon E3-1230 equipped with 16~GB RAM. In our network, the communication between various machines was bridged
using a 1 Gbps switch.
%\jianliu{describe how many processes (replicas) at most can we generate in our setup.}

Each client invokes operation in a closed loop, i.e., each client may have at most one pending operation.
We evaluate the peak throughput with respect to the server failure threshold $f$. We also evaluate the latency incurred in the investigated BFT protocols with respect to the attained throughput.

We measure peak throughput as follows. We require that the client performs back to back requests; we then increase the number of clients and requests in the system until
the aggregated throughput attained by all requests is saturated. The peak throughput is then computed as the maximum aggregated amount of requests (in bytes) that can be handled per second.

%Each data point in our plots is averaged over 10 independent measurements; where appropriate, we include the corresponding 95\% confidence intervals.
%as data objects.



\subsection{Evaluation Results}

\fig{fig:results} summarizes our evaluation results. We start by measuring the preprocessing performance in \BFT.
%We began our experiment by measuring the preprocessing time for \BFT.

%\vspace{0.5 em}
\noindent \textbf{Pre-processing performance: }\fig{fig:8} depicts the CPU time measured when generating shares for each counter with respect to the number of replicas.
Our results shows that the TEE only spends about 0.6~ms when generating shares for 20 replicas; this time increases linearly as $n$ increases (e.g., 1.6~ms for 200 replicas).
This also implies that it only takes several seconds to generate shares for thousands of counters (queries).
We therefore argue that the offline preprocessing will not create a bottleneck in \BFT. In what follows, we evaluate the online performance of \BFT.
%  and we focused on the online phase in the following experiments.

%\vspace{0.5 em}
\noindent \textbf{Impact of the reply payload size: }We start by evaluating the impact of the payload size on the latency incurred in different protocols with various payload sizes ranging from 1 byte to 1MB. Here, we set $n=103$ (which corresponds to our default network size). %since this is the average case in our setup.
\fig{fig:7} shows that \BFT achieves the lowest latency for all payload sizes. For instance, \BFT requires 4 ms for a reply payload size of 1~KB, which is 2 times faster than Zyzzyva.
Our findings also suggest that the latency is mainly affected by payload sizes that are larger than 1~KB (e.g., 1~MB). We speculate that this effect is mainly caused by the overhead of transmitting such large payloads in the system. Based on this observation, we proceed to evaluate the online performance of the investigated BFT protocols for payload sizes of 1 KB and 1 MB, respectively. Notice that the payload size plays an important role in determining the effective transactional throughput of a system. For instance, Bitcoin's consensus requires 600 seconds on average, but since payload size (block size) is 1~MB, Bitcoin can achieve a peak throughput of 7 transactions per second (each Bitcoin transaction is 250 Bytes on average).

%\vspace{0.5 em}
\noindent \textbf{Consensus performance: }\fig{fig:3} and~\ref{fig:6} evaluate the latency vs throughput exhibited by \BFT in comparison to other BFT variants for payload sizes 1~KB and 1~MB, respectively. Our results show that \BFT achieve the highest throughput while exhibiting the lowest average latency per operation. When the payload size is 1~KB, \BFT achieves a peak throughput of 490 operations per second, which is 4 times larger than CheapBFT. The superior performance of \BFT becomes even more pronounced as the payload size increases since \BFT exhibits very low communication overhead. In this case, \BFT achieves a peak throughput of 47 operations per second, which is 10 times larger than CheapBFT.
Assuming that each payload comprises transactions of 250 bytes (e.g., similar to Bitcoin), \BFT can process a maximum of 197,132 transactions per second when the network comprises \mbox{around 100 replicas}.
%\jianliu{I calculated as 28MB/256B, replace 28 with the right number.}

%\vspace{0.5 em}
\noindent\textbf{Impact of the network size: }\fig{fig:9} depicts the peak throughput achieved by different protocols with respect to the network size
for a 1~KB payload size, \BFT's performance is modest when compared to Zyzzyva and CheapBFT when the number $n$ of replicas is small. While the performance of these latter protocols degrades significantly as $n$ increases, \BFT's performance is marginally affected. For example, when $n=199$, \BFT achieves a peak throughput of 370 operations per second when compared to 56 and 38 op/s for Zyzzyva and CheapBFT, respectively. As mentioned earlier, as the payload size increases to 1~MB, \BFT's performance is even further exacerbated. \BFT is 20 times faster than Zyzzyva even for small networks where $n=19$.

%provides the lowest throughput for small $n$, but decreases slowly as $n$ increases.
%On the other hand, all other protocols decrease dramatically.
%For example, Zyzzyva provides the highest throughput for $n=20$, but was crossed by \BFT at $n=\X$.
%For 1MB payload size, \BFT provides the best throughput even at the beginning, and it is much higher than others (e.g., about \X times better than CheapBFT).


%\vspace{0.5 em}
\noindent \textbf{Scalability w.r.t. $f$: }Notice that comparing performance with respect to the number of replicas does not provide a fair basis to compare \BFT to those protocols that belong to the classical model. For instance, when $n=103$ replicas, Zyzzyva and PBFT can only tolerate $f=34$ faults, while \BFT, CheapBFT, and MinBFT can tolerate at most $f=51$ Byzantine failures.

To provide fair comparison, we evaluate the comparative performance of \BFT with respect to $f$ in Figures~\ref{fig:1},~\ref{fig:2},~\ref{fig:4}, and~\ref{fig:5}.
Our results confirm our findings in Section~\ref{sec:discussion} and show that \BFT establishes a strong tradeoff between performance and robustness.
% the maximum number of faults a protocol can tolerate.
%In this case, the superiority of \BFT over other protocols is shown more clearly ing
%We also measured the latency for various throughputs with a fixed $f=51$.





==> chapters/preliminaries_old.tex <==
%!TEX root = ../submission.tex
\section{Preliminaries}
\label{sec:preliminaries}

\remove{
\subsection{Notations}
A table of notations is shown in Table~\ref{notationtable}.

\begin{table}[h]
\begin{tabular}{|c|c|}
\hline
\textbf{Notation} & \textbf{Description} \\ \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Entities}} \\ \hline
$\Cli$       & Client                      \\ \hline
$\Ser$      & Replica                     \\ \hline
$\Ser_p$      & Primary                     \\ \hline
$\Ser_i$      & Backup                     \\ \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Objects}} \\ \hline
$M$ & Request message \\ \hline
$O$ & Execute history \\ \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Parameters}} \\ \hline
$n$ & Number of servers \\ \hline
$f$ & Number of faulty servers \\ \hline
$p$ & Primary number  \\ \hline
$v$  & View number  \\ \hline
$c$ & Counter value \\ \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Cryptographic Notations}} \\ \hline
$H()$               &    Cryptographic hash function \\ \hline
$h$               &     Cryptographic hash             \\ \hline
$E()$	& Authenticated encryption \\ \hline
$\sigma$     & Signature  \\ \hline

\end{tabular}
\caption{Summary of notations}
\label{notationtable}
\end{table}
}

\subsection{BFT for State Machine Replication}

\remove{
{\em Byzantine fault} was introduced to capture arbitrary behavior of a faulty process~\cite{Byzantine}.
For instance, an adversary can control the behavior of the compromised processes in order to cause the rest of the system to act in an erroneous way.
{\em Asynchrony} is a non-assumption about timing properties, i.e., there is no assumption about the processing speeds and transmission delays.
This (non-) assumption is realistic when the adversary fully controls the network.
}

It has been proved that consensus {\em cannot} be deterministically solved in an asynchronous system where a single faulty process exists.
This impossibility result is called Fischer-Lynch-Paterson, FLP, result~\cite{FLP}.
For decades, researchers have been struggling to circumvent this result.
One elegant solution was made by Castro and Liskov, who presented {\em practical Byzantine fault tolerance} (PBFT)
for {\em state machine replication} (SMR) services~\cite{PBFT}.
Such a service is modeled as a state machine that is replicated across different {\em replicas} $\Ser$s, 
and clients $\Cli$s send requests for some operations to it. 
PBFT guarantees that all non-faulty replicas agree on a total order for the execution of requests (i.e., {\em safety}),
and clients eventually receive replies to their requests (i.e., {\em liveness}).
PBFT does not rely on synchrony to provide safety, but it relies on {\em weak synchrony} to provide liveness.
Under a weak synchrony assumption, messages are guaranteed to be delivered after a certain time bound.
In PBFT, one replica called the {\em primary} $\Ser_p$ decides the order for clients' requests, and forwards them to others $\Ser_i$s.
However, $\Ser_p$ may be faulty, i.e., it may make conflicting statements which is called {\em equivocation}, or even stop processing requests.
Therefore $\Ser_i$s detect the misbehavior of $\Ser_p$ and trigger a {\em view-change} to select a new primary. 
The weak synchrony assumption guarantees that view-change will eventually happen.

Following PBFT, there are huge amount of work about improving the performance of SMR under the same assumption. 
Based on their message patterns, we roughly classify them into three categorizes:












%PBFT provides both {\em safety} and {\em liveness} if $n \geq 3f + 1$.
%Safety means that %the replicated service behaves like a centralized implementation that executes operations atomically one at a time,
%all non-faulty servers agree on a total order for the execution of requests despite failures, %Safety requires the bound on the number of faulty servers because a faulty server can behave arbitrarily, e.g., it can destroy its state.
%and liveness means clients eventually receive replies to their requests.
%PBFT does not rely on synchrony to provide safety, but it relies on {\em weak synchrony} to provide liveness.
%Under a weak synchrony assumption, messages are guaranteed to be delivered after a certain time bound.
%More precisely, the delay bound is time varying, but eventually does not grow faster than a polynomial function of time~\cite{partial_synchrony}.

In PBFT, replicas move through a succession of configurations called {\em views}.
In a view one replica is the {\em primary} $\Ser_p$ and the others $\Ser_i$ are {\em backups}.
$\Ser_p$ decides the order for clients' requested operations, and forwards them to $\Ser_i$s.
However, $\Ser_p$ may be faulty, i.e., it may make conflicting statements (which is called equivocation) or even stop processing requests.
Therefore $\Ser_i$s detect the misbehavior of $\Ser_p$ and trigger {\em view-changes} to select a new primary.

%t may assign the same sequence number to different requests, stop assigning sequence numbers, or leave gaps between sequence numbers.

PBFT uses a three phases protocol, i.e., {\em pre-prepare, prepare} and {\em commit} to order requests (across views). %sent in the same view and ensure that requests that commit  are totally ordered across views.
When $\Ser_p$ receives a request from $\Cli$, it assigns a sequence number to it and multicasts a $\preprepare$.
$\Ser_i$ accepts this $\preprepare$ provided it has not accepted another one with the same sequence number for a different message.
Then each $\Ser_i$ sends all other replicas a $\prepare$, which signals that $\Ser_i$ has agreed to assign the sequence number to this request.
Each replicas collects messages until it has received $2f$ $\prepare$s (including its own).
Next, each $\Ser_i$ multicasts a $\commit$ saying that it has been ready to execute.
After collecting $2f+1$ $\commit$s, each $\Ser_i$ executes the operation in the request and send a reply to $\Cli$,
who waits for $f+1$ consistent replies to accept the result.


\remove{
\subsection{Trusted Execution Environment}
\label{sub:sec:tee}

\jianliu{I copied this directly from our carousel paper.}
A \emph{Trusted Execution Environment} (TEE)~\cite{GP} is a system security primitive that isolates and protects security-critical logic from all other software on the platform.
All software outside TEE is said to be running in the \emph{Rich Execution Environment} (REE)~\cite{GP}, which usually includes the majority of the platform's software and the main operating system (OS).
A piece of application logic running inside TEE is referred to as a \emph{Trusted Application} (TA), whilst an application running in the REE is a \emph{Client Application} (CA)~\cite{GP}.

Fundamentally, a TEE provides confidentiality and integrity protection for TA's data, and ensures that no REE software can interfere with TA's operation.
A TEE usually provides some form of \emph{remote attestation}, which allows remote users to ascertain the current configuration and behavior of a TA.
The combination of these properties enables remote users to trust a TA.

In modern systems, the capability to establish and enforce a TEE is often provided by the CPU itself.
This provides very strong hardware-enforced security guarantees, and also allows the TEE to run on the main CPU, which is important in terms of performance and deployability.

Our approach does not depend on any platform-specific features, and thus can be realized on any TEE that exhibits the above characteristics.
We choose the recent \emph{Software Guard Extensions} (SGX) technology~\cite{SGX1} from Intel as the TEE in our implementation.
SGX allows individual applications to establish their own TEEs, called \emph{enclaves}.
An enclave can contain application logic and secret data, and protects the confidentially and integrity of its contents from all other software on the platform, including other enclaves, applications, or the (untrusted) OS.
SGX includes remote attestation capabilities to provide remote parties with assurance about the code running in an enclave~\cite{Anati2013}.

 }




\subsection{MinBFT}

Veronese et al. presented another SMR protocol called  MinBFT~\cite{MinBFT}.
Compared with PBFT, it reduces the number of required servers from $3f+1$ to $2f+1$ and the number of communication phases from 3 to 2.
They use a {\em trusted counter service} to prevent equivocation from faulty replicas.
Namely, they assume each replica holds a TEE that can sign a message together with a unique, monotonic and sequential counter value~$c$.


%TODO:reword
%These three properties imply that the USIG (1) will never assign the same identifier to two different messages (uniqueness), (2) will never assign an identifier that is lower than a previous one (monotonicity), and (3) will never assign an identifier that is not the successor of the previous one (sequentiality). These properties are guaranteed even if the server is compromised, so the service has to be implemented inside a TEE.
%------------

$\Ser_p$ assigns a sequence number to a request $M$ by requesting a signed counter value $\langle H(M), c_p\rangle_{\sigma_p}$ from its local $\TA$.
Since the counter is monotonic, $\Ser_p$ cannot assign the same counter value to another request,
and other replicas will not accept a larger counter value if they are expecting $c_p$ from $\Ser_p$.
Thus, $\Ser_p$ cannot do equivocation at this point.
$\Ser_p$ multicasts a $\prepare$ that contains $M$ and $\langle H(M), c_p\rangle_{\sigma_p}$ to all replicas.
Each $\Ser_i$ verifies this $\prepare$ and then multicasts a $\commit$ that contains $M$, $\langle H(M), c_p\rangle_{\sigma_p}$ and $\langle H(M), c_i\rangle_{\sigma_i}$,
where the last element is a signed counter value generated by its own $\TA$ and is used to guarantee that $\Ser_i$ cannot do equivocation during view-change.
After receiving $f+1$ $\commit$s, $\Ser_i$ executes the operation in $M$  and sends a reply to $\Cli$,
who waits for $f+1$ consistent replies to accept the result.

When $\Ser_p$ is faulty, a view-change has to be executed to choose a new primary $\Ser_{p'}$.
$\Ser_i$ who suspects that the primary is faulty starts a view-change by sending a $\reqviewchange$ to all replicas.
After receiving $f+1$ $\reqviewchange$s, $\Ser_i$ moves to the next view and multicasts $\viewchange$ that contains
the {\em execute history} $O$ which includes all $\prepare$s, $\commit$s, $\viewchange$s and $\newview$s sent by itself.
It also contains $\langle H(O), c_i\rangle_{\sigma_i}$ so that $\Ser_i$ cannot drop any message from $O$.
After receiving $f+1$ $\viewchange$ messages, the new primary $\Ser_{p'}$ multicasts a $\newview$ that contains all the $\viewchange$
messages received by $\Ser_{p'}$ plus the one sent by it.
Then each $\Ser_i$ executes the operations that have not been executed before, and switch to the new view.

Each replica needs to keep a vector with the highest counter value it received from each of the other replicas in $\prepare$,  $\commit$, $\checkpoint$ and $\viewchange$ messages.



\remove{
\jianliu{In \cite{Veronese2013}, they didn't say anything about the following situation: An honest server \Ser$_i$ multicasts a COMMIT message with a counter value $c$. Suppose some servers didn't receive this message, but they've received $f+1$ valid COMMIT messages. So they will still get an agreement in this round. But in next round, these servers will expect to receive a counter $c$ from \Ser$_i$, but this will never happen since the trusted hardware in \Ser$_i$ will only assign $c+1$.
 \\
 \\
New: it seems that there is even no need to include a counter in a COMMIT message. A signed counter in the PREPARE message is enough to guarantee the safety of the protocol.
}
}

\subsection{CheapBFT}

%In addition to using a trusted counter service,
CheapBFT~\cite{CheapBFT} also uses a composite agreement
where only $f+1$ active servers agree on and execute client requests during normal-case operation.
The other $f$ passive servers just modify their states by processing state updates provided by the active servers.
In case of suspected faulty behavior, CheapBFT triggers a transition protocol to activate the passive replicas, and then switch to MinBFT.

After receiving a request from $\Cli$, $\Ser_p$ constructs the same $\prepare$ as that is in MinBFT, but only multicasts it to active replicas.
Each active $\Ser_i$ does the same thing as MinBFT.
The only thing different is that after execution $\Ser_i$ not only sends $\reply$ to $\Cli$ but also to all passive replicas.
Each passive replica adjusts its sate after receiving $f+1$ $\reply$s.


In case of suspected faulty behavior of any active replica,
CheapBFT falls back to MinBFT using a transition protocol that is responsible for the safe protocol switch.
The suspecting replica sends a $\panic$ to all (active and passive) replicas.
The new primary $\Ser_{p'}$ sends a $\history$ message that contains the execute history $O$ and a signed counter to all replicas.
Upon receiving a $\history$ from $\Ser_{p'}$, it verifies it first, and then multicasts a $\switch$ that contains its own counter.
When $\Ser_i$ has obtained a correct history and $f$ matching $\switch$ messages from different replicas, the history becomes stable.
In this case, $\Ser_i$ processes the abort history, taking into account its local state.
Having processed the history, all non-faulty replicas are in a consistent state and therefore able to safely switch to MinBFT.




==> chapters/state.tex <==
%!TEX root = ../submission.tex
\section{BFT and Sate-of-the-Art}
\label{sec:states}

\remove{
\subsection{Notations}
A table of notations is shown in Table~\ref{notationtable}.

\begin{table}[h]
\begin{tabular}{|c|c|}
\hline
\textbf{Notation} & \textbf{Description} \\ \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Entities}} \\ \hline
$\Cli$       & Client                      \\ \hline
$\Ser$      & Replica                     \\ \hline
$\Ser_p$      & Primary                     \\ \hline
$\Ser_i$      & Backup                     \\ \hline
%USIG    &   Unique Sequential Identifier Generator  \\ \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Objects}} \\ \hline
$M$ & Request message \\ \hline
$O$ & Execute history \\ \hline
%$\UI$	     &   Unique Identifier    \\ \hline
%$N$         &   Ephemeral nonce    \\  \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Parameters}} \\ \hline
$n$ & Number of servers \\ \hline
$f$ & Number of faulty servers \\ \hline
$p$ & Primary number  \\ \hline
$v$  & View number  \\ \hline
$c$ & Counter value \\ \hline

\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Cryptographic Notations}} \\ \hline
$H()$               &    Cryptographic hash function \\ \hline
$h$               &     Cryptographic hash             \\ \hline
$E()$	& Authenticated encryption \\ \hline
$\sigma$     & Signature  \\ \hline
%$x$               &     Secret (signing) key            \\ \hline
%$X$               &     Public (verification) key            \\ \hline

\end{tabular}
\caption{Summary of notations}
\label{notationtable}
\end{table}
}

{\em Byzantine fault} was introduced to capture arbitrary behavior of a faulty process~\cite{Byzantine}.
For instance, an adversary can control the behavior of the compromised processes in order to cause the rest of the system to act in an erroneous way.
{\em Asynchrony} is a non-assumption about timing properties, i.e., there is no assumption about the processing speeds and transmission delays.
This (non-) assumption is realistic when the adversary fully controls the network.
It has been proved that consensus {\em cannot} be deterministically solved in an asynchronous system where a single process can crash.
This impossibility result is called Fischer-Lynch-Paterson, FLP, result~\cite{FLP}.

For decades, people has been struggling to circumvent this result.
One elegant solution was made by Castro and Liskov, who presented {\em practical Byzantine fault tolerance} (PBFT)
for {\em state machine replication} (SMR) services~\cite{PBFT}.
Such a service is modeled as a state machine that is replicated across different {\em replicas}, 
and clients send requests for some operations to the replicas.
\TODO{one sentence about the relation between BFT and SMR}
PBFT guarantees that all non-faulty replicas agree on a total order for the execution of requests (i.e., {\em safety}),
and clients eventually receive replies to their requests (i.e., {\em liveness}).
PBFT does not rely on synchrony to provide safety, but it relies on {\em weak synchrony} to provide liveness.
Under a weak synchrony assumption, messages are guaranteed to be delivered after a certain time bound.
More precisely, the delay bound is time varying, but eventually does not grow faster than a polynomial function of time~\cite{partial_synchrony}. 
In the {\em normal case} of PBFT, one replica that is called the {\em primary} $\Ser_p$ decides the order for clients' requests, and forwards them to others $\Ser_i$s.
However, $\Ser_p$ may be faulty, i.e., it may make conflicting statements which is called {\em equivocation}, or even stop processing requests.
Therefore $\Ser_i$s detect the misbehavior of $\Ser_p$ and trigger a {\em view-change} to select a new primary. 
The weak synchrony assumption guarantees that view-change will eventually happen.

Following PBFT, there are huge amount of work about improving the performance of SMR under the same assumption. 
Based on their message patterns, we roughly classify them into three categorizes:

\noindent{\bf Classic.}
%PBFT uses a three phases protocol, i.e., {\em pre-prepare, prepare} and {\em commit} to order requests (across views). %sent in the same view and ensure that requests that commit  are totally ordered across views.
In PBFT, when $\Ser_p$ receives a request from $\Cli$, it assigns a sequence number to it and multicasts a $\preprepare$.
$\Ser_i$ accepts this $\preprepare$ if it has not accepted another one with the same sequence number for a different message.
Then each $\Ser_i$ sends all other replicas a $\prepare$, which signals that $\Ser_i$ has agreed to assign the sequence number to this request.
Each replicas collects messages until it has received $2f$ $\prepare$s (including its own).
Next, each $\Ser_i$ multicasts a $\commit$ saying that it has been ready to execute.
After collecting $2f+1$ $\commit$s, each $\Ser_i$ executes the operation in the request and send a reply to $\Cli$,
who waits for $f+1$ consistent replies to accept the result.
We call BFT protocols that follow this kind of message pattern as {\em classic} BFT. 

Veronese et al. presented another classic BFT protocol called  MinBFT~\cite{MinBFT}.
Compared with PBFT, it reduces the number of required servers from $3f+1$ to $2f+1$ and the number of communication phases from 3 to 2.
They use a {\em trusted counter service} to prevent equivocation from faulty replicas.
Namely, they assume each replica holds a TEE that can sign a message together with a unique, monotonic and sequential counter value~$c$.
$\Ser_p$ assigns a sequence number to a request $M$ by requesting a signed counter value $\langle H(M), c_p\rangle_{\sigma_p}$ from its local $\TA$.
Since the counter is monotonic, $\Ser_p$ cannot assign the same counter value to another request,
and other replicas will not accept a larger counter value if they are expecting $c_p$ from $\Ser_p$.
Thus, $\Ser_p$ cannot do equivocation at this point.
$\Ser_p$ multicasts a $\prepare$ that contains $M$ and $\langle H(M), c_p\rangle_{\sigma_p}$ to all replicas.
Each $\Ser_i$ verifies this $\prepare$ and then multicasts a $\commit$ that contains $\langle H(M), c_p\rangle_{\sigma_p}$ and $\langle H(M), c_i\rangle_{\sigma_i}$,
where the second element is a signed counter value generated by its own $\TA$ and is used to guarantee that $\Ser_i$ cannot do equivocation during view-change.
%After receiving $f+1$ $\commit$s, $\Ser_i$ executes the operation in $M$  and sends a reply to $\Cli$,
%who waits for $f+1$ consistent replies to accept the result.

\remove{
When $\Ser_p$ is faulty, a view-change has to be executed to choose a new primary $\Ser_{p'}$.
$\Ser_i$ who suspects that the primary is faulty starts a view-change by sending a $\reqviewchange$ to all replicas.
After receiving $f+1$ $\reqviewchange$s, $\Ser_i$ moves to the next view and multicasts $\viewchange$ that contains
the {\em execute history} $O$ which includes all $\prepare$s, $\commit$s, $\viewchange$s and $\newview$s sent by itself.
It also contains $\langle H(O), c_i\rangle_{\sigma_i}$ so that $\Ser_i$ cannot drop any message from $O$.
After receiving $f+1$ $\viewchange$ messages, the new primary $\Ser_{p'}$ multicasts a $\newview$ that contains all the $\viewchange$
messages received by $\Ser_{p'}$ plus the one sent by it.
Then each $\Ser_i$ executes the operations that have not been executed before, and switch to the new view.

Each replica needs to keep a vector with the highest counter value it received from each of the other replicas in $\prepare$,  $\commit$, $\checkpoint$ and $\viewchange$ messages.
}

\noindent{\bf Speculative.}
Kotla et al. present Zyzzyva~\cite{Zyzzyva} that uses speculation to improve the performance of BFT.   
Unlike classic BFT, replicas in Zyzzyva execute $\Cli$s' requests following the order proposed by $\Ser_p$, without running any agreement protocol. 
After execution, they reply immediately to $\Cli$. 
If $\Ser_p$ is faulty and performs equivocation, $\Cli$ will receive inconsistent replies. 
In this case,  $\Cli$ help correct replicas recover from the inconsistent states.
Zyzzyva is able to reduce the overhead of SMR to near its theoretical minima. 
%and to achieve throughputs of tens of thousands of requests per second.
BFT protocols following this message pattern is called {\em speculative} BFT.

Similar to MinBFT, MinZyzzyva uses trusted counter to constrain the behavior of $\Ser_p$, allowing a reduction of the number of replicas from $3f+1$ to $2f+1$~\cite{MinBFT}. ... \cite{Next700} ...

\noindent{\bf Optimistic.}
Yin et al. propose a new BFT replication architecture that separates agreement that orders requests from execution that processes requests~\cite{Yin}. 
Replicas are separated into agreement cluster and execution cluster. 
%The agreement cluster's job is to order request and send them to the execution cluster. 

CheapBFT~\cite{CheapBFT} was built on this idea. 
It requires $f+1$ active replicas to agree on clients' requests during normal case operation.
The other $f$ passive servers just modify their states by processing state updates provided by the active replicas.
After receiving a request from $\Cli$, $\Ser_p$ constructs the same $\prepare$ as that is in MinBFT, but only multicasts it to active replicas.
Each active $\Ser_i$ does the same thing as MinBFT.
After execution, $\Ser_i$ not only sends $\reply$ to $\Cli$ but also to all passive replicas.
Each passive replica adjusts its sate after receiving $f+1$ $\reply$s.
In case of suspected faulty behavior of any active replica, CheapBFT triggers a transition protocol to activate the passive replicas, and then switch to MinBFT.
\remove{
In case of suspected faulty behavior of any active replica,
CheapBFT falls back to MinBFT using a transition protocol that is responsible for the safe protocol switch.
The suspecting replica sends a $\panic$ to all (active and passive) replicas.
The new primary $\Ser_{p'}$ sends a $\history$ message that contains the execute history $O$ and a signed counter to all replicas.
Upon receiving a $\history$ from $\Ser_{p'}$, it verifies it first, and then multicasts a $\switch$ that contains its own counter.
When $\Ser_i$ has obtained a correct history and $f$ matching $\switch$ messages from different replicas, the history becomes stable.
In this case, $\Ser_i$ processes the abort history, taking into account its local state.
Having processed the history, all non-faulty replicas are in a consistent state and therefore able to safely switch to MinBFT.
}
...\cite{XFT}...

In such protocols, only a subset of replicas are required to run the agreement protocol, and other replicas are required get involved only when failure happens. We call BFT protocols that follows this kind of message pattern as {\em optimistic} BFT.
Note that it is different from speculative BFT, where agreement is not required at all in normal case.

\noindent{\bf Comparisons.} 
We propose to compare BFT protocols in two dimensions:
\begin{itemize}
\item {\bf Performance:} time required to complete a request in normal case;
\item {\bf Robustness:} cost required to recover from non-primary faults
\footnote{All BFT protocols require view change to recover from primary faults, 
and this operation takes similar cost among different protocols.
So we only consider non-primary faults in terms of robustness.}.
\end{itemize}


Clearly, speculative BFT provides the best performance among these three categories since it avoids all-to-all broadcast.
However, the speculative execution cannot tolerate even a single crash fault, 
and the client needs to help correct replicas to converge on a single ordering of requests. 
In real-world scenarios, clients may have neither incentives nor computing power (e.g., lightweight clients) to get involved in the protocol.
If a (faulty) client fails to report the inconsistency, replicas whose state has diverged from others may not discover this fact.
Furthermore, if inconsistency appears, replicas may have to rollback some executions, which makes the programming model more complicated. 
Therefore, speculative BFT provides worst robustness.

In contrast, classic BFT can tolerate non-primary faults for free, but requires all replicas to get involved in the agreement protocol. 
So it provides best robustness but worst performance. 

Optimistic BFT is in the middle. It only requires active replicas to run the agreement protocol, which significantly reduce the message complexity but still requires all-to-all broadcast. 
It needs to run a transition protocol or view change to tolerate non-primary faults.
However, it does not require clients' help and there is no need to rollback.

